Assessing the Human Likeness of AI-Generated Counterspeech

Counterspeech is a targeted response to counteract and challenge abusive or hateful content. It effectively curbs the spread of hatred and fosters constructive online communication. Previous studies have proposed different strategies for automatically generated counterspeech. Evaluations, however, focus on relevance, surface form, and other shallow linguistic characteristics. This paper investigates the human likeness of AI-generated counterspeech, a critical factor influencing effectiveness. We implement and evaluate several LLM-based generation strategies, and discover that AI-generated and human-written counterspeech can be easily distinguished by both simple classifiers and humans. Further, we reveal differences in linguistic characteristics, politeness, and specificity. The dataset used in this study is publicly available for further research.

==> table.tex <==

%%Start Table
\begin{table}[b]
\centering
\scalebox{0.7}{
\begin{tabular}{lcccc}
\hline
                  & Prompt & Select & Constrained & Fine-tune \\ \hline
Agreement Rate    & 97\%   & 97\%   & 97\%        & 94\%      \\
Cohen Kappa Score & 0.94   & 0.94   & 0.93        & 0.88      \\ \hline
\end{tabular}}
\caption{Reliability in human likeness evaluation}
\label{Table: human likeness reliability}
\end{table}
%%End Table


%% Start Table 
\begin{table}[H]
\centering
\scalebox{0.6}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
                  & Prompt   & Select   & Constrained   & Fine-tune   & User & Expert \\ \midrule
Cohen Kappa Score & 0.80 & 0.94 & 0.96 & 0.93 & 0.80 & 0.88   \\ \bottomrule
\end{tabular}}
\caption{Reliability in politeness evaluation}
\label{Table: politeness reliability}
\end{table}
%% End Table 



% Start Table
\begin{table}[H]
\centering
\scalebox{0.6}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
                  & Prompt & Select & Constrained & Fine-tune & User & Expert \\ \midrule
Cohen Kappa Score & 0.87   & 0.86   & 0.80        & 0.95      & 0.93 & 0.81   \\ \bottomrule
\end{tabular}}
\caption{Reliability in suitableness evaluation}
\label{Table: suitableness reliability}
\end{table}
% End Table



% Start Table 
\begin{table}[b]
\centering
\scalebox{0.6}{
\begin{tabular}{lccccccccc}
\hline
\multirow{2}{*}{Strategies} & \multicolumn{3}{c}{AI}                 & \multicolumn{3}{c}{Human}                   & \multicolumn{3}{c}{Weight Average}            \\ \cline{2-10} 
                            & P             & R             & F1             & P             & R             & F1            & P             & R             & F1            \\ \hline
Fine-tune      & 0.80  & 0.95 & \textbf{0.87} & 0.94 & 0.76 & \textbf{0.84} & 0.87 & 0.86 & \textbf{0.86} \\ \hline
Constrained                    & 0.99            & 1.00              & 1.00              & 1.00              & 0.99              & 1.00              & 1.00              & 1.00              & 1.00              \\ \hline
Prompt         & 0.99          & 1.00              & 0.99          & 1.00              & 0.99          & 0.99          & 0.99          & 0.99          & 0.99          \\ \hline
Select              & 0.98          & 1.00              & 0.99          & 1.00              & 0.98          & 0.99          & 0.99          & 0.99          & 0.99          \\ \hline
Combined           & 0.95 & 1.00     & 0.97 & 1.00     & 0.95 & 0.97 & 0.98 & 0.97 & 0.97 \\ \hline
\end{tabular}}
\caption{Model performance of differentiating AI-generated counterspeech and human-written counterspeech across different methods. Fine-tune here indicates the experiment distinguishes counterspeech generated by Fine-tune from human-written counterspeech. Combined, this indicates the experiment of differentiating all the human-written counterspeech and AI-generated counterspeech.}
\label{Table: Model Performanc1}
\end{table}
% End Table




% Start Table 
\begin{table}[]
\centering
\scalebox{0.6}{

\begin{tabular}{@{}lccccccccc@{}}
\toprule
\multirow{2}{*}{Strategies} & \multicolumn{3}{c}{AI}      & \multicolumn{3}{c}{Human}   & \multicolumn{3}{c}{Weight Average} \\ \cmidrule(l){2-10} 
                            & P    & R    & F1            & P    & R    & F1            & P       & R      & F1              \\ \midrule
CONAN                       & 0.97 & 0.98 & 0.97          & 0.98 & 0.96 & 0.97          & 0.97    & 0.97   & 0.97            \\
Gab                         & 0.86 & 0.99 & 0.92          & 0.99 & 0.84 & 0.91          & 0.93    & 0.92   & 0.92            \\
Reddit                     & 0.81 & 0.95 & \textbf{0.88} & 0.94 & 0.78 & \textbf{0.85} & 0.88    & 0.87   & \textbf{0.87}   \\
Multi                       & 0.92 & 0.99 & 0.95          & 0.99 & 0.91 & 0.95          & 0.95    & 0.95   & 0.95            \\
Effectiveness               & 0.96 & 0.98 & 0.97          & 0.98 & 0.96 & 0.97          & 0.97    & 0.97   & 0.97            \\ \bottomrule
\end{tabular}}

\caption{Model performance of differentiating AI-generated counterspeech and human-written counterspeech across different specific Fine-tune methods. Fine-tune strategies utilize different datasets to fine-tune Llama, such as Benchmark Reddit, Benchmark Gab, Benchmark CONAN, and MultiCONAN, also the effective outcome dataset}
\label{Table: Model Performanc2}
\end{table}
% End Table 




%% Start Table 
\begin{table}[b]
\centering
\scalebox{0.6}{
\begin{tabular}{llllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Strategies}} & \multicolumn{3}{c}{AI} & \multicolumn{3}{l}{Human} & \multicolumn{3}{l}{Weight Average} \\ \cline{2-10} 
\multicolumn{1}{c}{}                           & P      & R     & F1    & P       & R      & F1     & P          & R         & F1        \\ \hline
Prompt                                             & 0.91   & 1.00  & 0.95  & 1.00    & 0.93   & 0.97   & 0.96       & 0.96      & 0.96      \\
Select                                             & 1.00   & 0.92  & 0.96  & 0.93    & 1.00   & 0.96   & 0.96       & 0.96      & 0.96      \\
Constrained                                             & 0.90   & 0.98  & 0.94  & 0.98    & 0.91   & 0.94   & 0.94       & 0.94      & 0.94      \\
Fine-tune                                             & 0.49   & 0.64  & \textbf{0.55}  & 0.63    & 0.48   & \textbf{0.55}   & 0.57       & 0.55      & \textbf{0.55}      \\ \hline
\end{tabular}}
\caption{Human performance in identifying Authorship}
\label{Tabel: Human performance}
\end{table}
%% End Table 





% Start: Table 
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table*}
\centering
\resizebox{1\textwidth}{!}{
	\setlength{\tabcolsep}{.075in}
	\centering
	\tiny
\begin{tabular}{l P{.5in}P{.5in}P{.5in}P{.5in}P{.5in}P{.5in}}
\hline
Category                                                                       & Prompt                           & Select                    & Constrained                        & Fine-tune                  & All                              \\ \hline
\textbf{Textual factors}                                                       &                                  &                                  &                                  &                                  &                                  \\
~~~1st person pronouns          & $\uparrow\uparrow$               & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ \\
~~~Action words                 & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       \\
~~~Format words                 & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Certainty words              & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ \\
~~~Frequency words              & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Self-Expression words        & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ \\
~~~Anticipation words           & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ \\
~~~Overstated Words             & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       \\ \hline
\textbf{Emotional factors}                                                     & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Support and affiliation      & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Excite from pleasure or pain & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Negative                     & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ \\
~~~Positive Words               & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Hatred                       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\ \hline
\textbf{Social related factors}                                                        & $\downarrow\downarrow\downarrow$ & $\downarrow\downarrow\downarrow$ & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\downarrow\downarrow\downarrow$ \\
~~~Religious words              & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Economic Words               & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Respect                      & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Wealth                       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\
~~~Power                        & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       & $\uparrow\uparrow\uparrow$       \\ \hline
\end{tabular}}
\caption{Linguistic analysis comparing counterspeech generated by AI and humans across different AI-based generation methods. The up arrow indicates higher values in human-written counterspeech. The number of arrows indicates the p-value of the Wilcoxon rank-sum test (one: $p<0.05$, two: $p<0.01$, and three: $p<0.001$). All tests have passed Bonferroni correction.}
\label{Table: Linguistic analysis}
\end{table*}
% End: Table 
